Online Data-Driven Safety Certification for Systems Subject to Unknown Disturbances

Deploying autonomous systems in safety critical settings necessitates methods to verify their safety properties. This is challenging because real-world systems may be subject to disturbances that affect their performance, but are unknown a priori. This work develops a safety-verification strategy wherein data is collected online and incorporated into a reachability analysis approach to check in real-time that the system avoids dangerous regions of the state space. Specifically, we employ an optimization-based moving horizon estimator (MHE) to characterize the disturbance affecting the system, which is incorporated into an online reachability calculation. Reachable sets are calculated using a computational graph analysis tool to predict the possible future states of the system and verify that they satisfy safety constraints. We include theoretical arguments proving our approach generates reachable sets that bound the future states of the system, as well as numerical results demonstrating how it can be used for safety verification. Finally, we present results from hardware experiments demonstrating our approach's ability to perform online reachability calculations for an unmanned surface vehicle subject to currents and actuator failures.

==> extra.tex <==
\begin{figure}
\centering
    \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\textwidth]{figures/numerical_results/one_step_double_int.eps}
        \caption{Forward reachability strategy for collision avoidance}
        % \label{fig:forward_reach_comp}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\textwidth]{figures/numerical_results/n_step_double_int.eps}
        \caption{Forward reachability strategy for collision avoidance}
        % \label{fig:forward_reach_comp}
    \end{subfigure}
    \caption{Comparison of different approaches to reachability analysis for safety certification in a collision avoidance scenario}
    %\label{fig:reach_comparison}
\end{figure}

{\color{blue}
\cref{fig:reach_comparison} also highlights the need to \emph{overapproximate} the backprojection, because an underapproximation would allow for states outside the backprojection to collide with an obstacle, eliminating the soundness of the safety certification. Note that this is in contrast to goal-checking as is considered in \cite{everett2021reachability} wherein backprojection underapproximations are required to guarantee that \emph{all} states in the backprojection estimate terminate in the target set.

Alternatively, reachability analysis can be conducted in reverse to compute \emph{backprojection sets}, which designate regions of a state space for which the NN control policy will drive the system to a \emph{target set}. To guarantee safety using backward reachability analysis, the target set can be configured to bound the avoid sets and the system is guaranteed to be safe as long as its state doesn't intersect with any backprojection sets, i.e., the system does not occupy a region that will lead to an avoid set.
While many studies have focused on forward reachability analysis, there are scenarios where it is a poor strategy for guaranteeing the safety of an NFL. Fig. \ref{fig:reach_comparison} shows a comparison between forward and backward reachability approaches for a hypothetical collision-avoidance scenario with a ground robot. In this case, the vehicle is approaching an obstacle in such a way that small perturbations in its position determine which direction it will take. As shown in Fig \ref{fig:forward_reach_comp}, forward reachability analysis will incorrectly anticipate a collision because the reachable set estimates span the two possible trajectories.
}

\nr{TODO: Move the theoretical stuff from this paragraph to approach section and clean up. Can still talk about how the new corollary can be used to improve efficiency in case of \cref{fig:backward_reach_single_integrator}}
The observation that the backprojection sets shrink into the target set in an obstacle avoidance scenario highlights an additional computational advantage of using a backward reachability strategy.
If $\bar{\mathcal{P}}_{-1}(\mathcal{X}_T) \subseteq \mathcal{X}_T$, then $\mathcal{P}_{-i}(\mathcal{X}_T) \subseteq \mathcal{X}_T\ \forall i \in [\tau]$ which means that at iteration $i$, we can throw out $\bar{\mathcal{P}}_{-i}(\mathcal{X}_T) \cup \mathcal{X}_T$. 
If for some $k<\tau$, $\bar{\mathcal{P}}_{-k}(\mathcal{X}_T) \subseteq \mathcal{X}_T$ then we do not need to calculate the remaining backprojections.
Additionally, if $X_0 \cup \bar{\mathcal{P}}_{-k:0}(\mathcal{X}_T) = \emptyset$, $X_0$ is guaranteed safe for an infinite time horizon.

\textcolor{blue}{
\cref{thm:backprojection} provides a formula for computing $\bar{\mathcal{P}}_{-1}(\mathcal{X}_T)$, i.e., an under-approximation of the backprojection set for a single timestep.
This section extends that idea to enable computing $\bar{\mathcal{P}}_{-\tau:0}(\mathcal{X}_T)$ for a time horizon $\tau$ and also describes how partitioning can help improve the results, particularly when \cref{eqn:backreachable:polytope} is the empty set.
The proposed procedure is summarized in~\cref{alg:backprojection}.
}

\textcolor{blue}{
After initializing the zeroth backprojection set as the target set (\cref{alg:backprojection:initialize}), we recursively compute $\bar{\mathcal{P}}_{t}(\mathcal{X}_T)$ backward in time (\cref{alg:backprojection:timestep_for_loop}).
For each timestep, we first compute an over-approximation on the backreachable set, $\bar{\mathcal{R}}^B_{t}(\mathcal{X}_T)$, by solving the LPs in \cref{eqn:backreachable:lpmax_obj,eqn:backreachable:lpmax_constr_control,eqn:backreachable:lpmax_constr_state} and \cref{eqn:backreachable:lpmin_obj,eqn:backreachable:lpmin_constr_control,eqn:backreachable:lpmin_constr_state} (\cref{alg:backprojection:backreach}).
}

\textcolor{blue}{
Since $\mathcal{R}^B_{t}(\mathcal{X}_T) \supseteq \mathcal{P}_{t}(\mathcal{X}_T)$, we can relax the NN over $\mathcal{R}^B_{t}(\mathcal{X}_T)$, and that relaxation will also hold for all states in $\mathcal{P}_{t}(\mathcal{X}_T)$ and $\bar{\mathcal{P}}_{t}(\mathcal{X}_T)$.
However, $\mathcal{R}^B_{t}(\mathcal{X}_T)$ could be large, which could lead to a loose NN relaxation.
Thus, instead of analyzing $\mathcal{R}^B_{t}(\mathcal{X}_T)$ as a single set, we uniformly partition the set $\mathcal{R}^B_{t}(\mathcal{X}_T)$ into $\mathbf{r}\in\mathds{N}^{n_x}$ cells (defined per dimension).
}

\textcolor{blue}{
For each cell in the partition, we have a (hyper-)rectangular set of states, $[\ubar{\mathbf{x}}_{t}, \bar{\mathbf{x}}_{t}]_i$, that could be passed as inputs to the NN controller.
The NN can be relaxed over this set using CROWN (\cref{thm:crown_particular_x}) or a similar type of algorithm.
In particular, we extract $\CROWNAu, \CROWNAl, \CROWNbu, \CROWNbl$ from CROWN, which define $\mathbf{P}$ and $\mathbf{p}$, the constraints in \cref{eqn:backreachable:polytope} (\cref{alg:backprojection:polytope_constraint_A,alg:backprojection:polytope_constraint_b}).
These constraints define a polytope of states that are guaranteed to lead to $\bar{\mathcal{P}}_{t+1}(\mathcal{X}_T)$ at the next timestep (for any control within CROWN's bounds), so those states should be added to $\bar{\mathcal{P}}_{t}(\mathcal{X}_T)$ (\cref{alg:backprojection:union}).
Note that it is possible, despite partitioning, that $\mathcal{A}=\emptyset$.
After following this procedure for each timestep, the algorithm returns a sequence of inner-approximations of the backprojection sets (\cref{alg:backprojection:return}).
}

==> related_work.tex <==
%!TEX root=main.tex

\section{Related Work}

